Overview of Speaker Modeling and Its Applications: From the Lens of Deep Speaker Representation Learning

Speaker individuality information is among the most critical elements within speech signals. By thoroughly and accurately modeling this information, it can be utilized in various intelligent speech applications, such as speaker recognition, speaker diarization, speech synthesis, and target speaker extraction. In this overview, we present a comprehensive review of neural approaches to speaker representation learning from both theoretical and practical perspectives. Theoretically, we discuss speaker encoders ranging from supervised to self-supervised learning algorithms, standalone models to large pretrained models, pure speaker embedding learning to joint optimization with downstream tasks, and efforts toward interpretability. Practically, we systematically examine approaches for robustness and effectiveness, introduce and compare various open-source toolkits in the field. Through the systematic and comprehensive review of the relevant literature, research activities, and resources, we provide a clear reference for researchers in the speaker characterization and modeling field, as well as for those who wish to apply speaker modeling techniques to specific downstream tasks.

==> figs/overview/organization.tex <==
\begin{tikzpicture}[node distance=2cm, auto, thick, main node/.style={circle, draw, minimum size=1cm, inner sep=0pt}]

% 定义节点
\node[main node] (sec1) {Sec. 2: Key Components in TTS};
\node[main node, below=of sec1] (sec21) {Sec. 2.1: Main Taxonomy};
\node[main node, below left=of sec21] (sec22) {Sec. 2.2: Text Analysis};
\node[main node, below right=of sec21] (sec23) {Sec. 2.3: Acoustic Model};
\node[main node, below=of sec23] (sec24) {Sec. 2.4: Vocoder};
\node[main node, below=of sec24] (sec25) {Sec. 2.5: Towards Fully E2E TTS};
\node[main node, below=of sec25] (sec26) {Sec. 2.6: Other Taxonomies};

% 定义子节点
\node[main node] at ($(sec1.south)!0.5!(sec21.north)$) (sec3) {Sec. 3: Advanced Topics in TTS};
\node[main node] at ($(sec3.south)!0.5!(sec21.north)$) (sec4) {Sec. 4: Resources};

% 绘制连接线
\path[->, >=stealth] (sec1) edge (sec21)
                      (sec21) edge (sec22)
                      (sec21) edge (sec23)
                      (sec23) edge (sec24)
                      (sec24) edge (sec25)
                      (sec25) edge (sec26)
                      (sec3) edge (sec21)
                      (sec4) edge (sec21);

\end{tikzpicture}
